Feature Decomposition for Reducing Negative Transfer: A Novel Multi-task Learning Method for Recommender System

In recent years, thanks to the rapid development of deep learning (DL), DL-based multi-task learning (MTL) has made significant progress, and it has been successfully applied to recommendation systems (RS). However, in a recommender system, the correlations among the involved tasks are complex. Therefore, the existing MTL models designed for RS suffer from negative transfer to different degrees, which will injure optimization in MTL. We find that the root cause of negative transfer is feature redundancy that features learned for different tasks interfere with each other. To alleviate the issue of negative transfer, we propose a novel multi-task learning method termed Feature Decomposition Network (FDN). The key idea of the proposed FDN is reducing the phenomenon of feature redundancy by explicitly decomposing features into task-specific features and task-shared features with carefully designed constraints. We demonstrate the effectiveness of the proposed method on two datasets, a synthetic dataset and a public datasets (i.e., Ali-CCP). Experimental results show that our proposed FDN can outperform the state-of-the-art (SOTA) methods by a noticeable margin.

==> LaTeX 3/Abstract.tex <==
\begin{abstract}
 In recent years, thanks to the rapid development of deep learning (DL), DL-based multi-task learning (MTL) has made significant progress, and it has been successfully applied to recommendation systems (RS). However, in a recommender system, the correlations among the involved tasks are complex. Therefore, the existing MTL models designed for RS suffer from \textit{negative transfer} to different degrees, which will injure optimization in MTL. We find that the root cause of negative transfer is \textit{feature redundancy} that features learned for different tasks interfere with each other.
%that is the learned task-specific feature space contains other unnecessary features.
%due to the complexity of the recommendation system, the current state-of-the-art multi-task learning models still has different degrees of negative transfer problems. This may be because when the model performs feature transformation on the original input, it only makes a corresponding strategy for parameter sharing, and does not explicitly split the original features, resulting in the model after multiple iterations, the task-specific space still exists shared features, and the shared feature space still contain some task-specific features. 
To alleviate the issue of negative transfer, we propose a novel multi-task learning method termed Feature Decomposition Network (FDN). The key idea of the proposed FDN is reducing the phenomenon of feature redundancy by explicitly decomposing features into task-specific features and task-shared features with carefully designed constraints. %\textcolor{red}{The key idea of the proposed FDN is reducing the complexity of tasks' correlations by explicitly decomposing features into task-specific features and task-shared features with carefully designed constraints. The decomposed features are then recombined based on the requirements so that the final features used for each task can be more representative.}
% 上述标红原因是这句话主要描述的是减少任务复杂性，但是正文没有减少任务复杂性的体现，是否需要改为减少特征冗余现象？The key idea of the proposed FDN is reducing the phenomenon of feature redundancy by explicitly decomposing features into task-specific features and task-shared features with carefully designed constraints. 
%With carefully-designed constraints, our model can effectively decompose features. 
%Besides, an ensemble model is adopted to improve the expressivity of the recombined features.  
%the private and shared features of the task when extracting features from the original input, which avoids the problem of negative transfer caused by the above reasons during the training process. 
% We demonstrate the effectiveness of the proposed method on three datasets, a synthetic dataset and two public datasets (i.e., \textit{Ali-CCP} and \textit{Census-Income}). Experimental results show that our proposed FDN can outperform the state-of-the-art (SOTA) methods by a noticeable margin.
We demonstrate the effectiveness of the proposed method on two datasets, a synthetic dataset and a public datasets (i.e., \textit{Ali-CCP}). Experimental results show that our proposed FDN can outperform the state-of-the-art (SOTA) methods by a noticeable margin.
\end{abstract}

==> LaTeX 3/Conclusion.tex <==
\section{Conclusion}
In this paper, we have proposed a novel multi-task learning method, called FDN, for recommender system. The core of the FDN is a new feature decomposition module with two carefully-designed constraints. Besides, an ensemble model is adopted to further improve the expressivity of the extracted feature.
%, this module can extract decomposed features, i.e., task-shared feature and task-private feature, which can effectively relieve the issue of negative transfer by reducing feature interference. 
We have conducted experiments on two datasets and achieved new SOTA performance.
%to demonstrate the effectiveness of the new model. In our future study, we will explore how to decompose the feature space in multi-layer feature extraction models, which is similar to ML-MMoE and PLE. 
%In our future study, how to effectively decompose the feature space in multi-layer feature extraction models based on ML-MMoE and PLE.

==> LaTeX 3/Experiment.tex <==
\section{Experiments on Ali-CCP Dataset}

To demonstrate the effectiveness of the newly proposed FDN, we conducted experiments on ``Alibaba Click and Conversion Prediction'' (Ali-CCP). We take MMoE \cite{ma2018modeling} as the baseline model, and also compare FDN with the SOTA models, CGC and PLE \cite{tang2020progressive}. %In the experiment, MMoE and CGC are set with 8 experts, and PLE is set with 2 layers and 16 experts. Our model is set with 2 DCPs for each task.
% To demonstrate the effectiveness of the newly proposed FDN, we conducted experiments on two public datasets. We take MMoE \cite{ma2018modeling} as the baseline model, and also compare FDN with the state-of-the-art models, CGC and PLE \cite{tang2020progressive}. In the experiment, MMoE and CGC are set with 8 experts, and PLE is set with 2 layers and 16 experts. Our model is set with 2 DCPs for each task. % \chuan{Why use these hyper-parameters? You should also tell the reason here.}.
% \textcolor{red}{need to explain more about these three baseline models if we have space.}
% Like "The MMoE and CGC models have 8 experts, and PLE has 2 layers and 16 experts. Our model is set 2 modules in each task".

%In order to verify the effectiveness of the FDN, we conducted experiments on public Ali-CCP dataset and  real business scenarios (Xiaomi Radio Recommendation). We take MMoE as the baseline model, and compare CGC and PLE \cite{tang2020progressive}, the state-of-the-art multi-task learning proposed by Tencent. We do a comparative experiment on offline and online business indicators.

% \subsection{Ali-CCP Dataset}

%In this subsection, we have done some experiments on "Alibaba Click and Conversion Prediction (Ali-CCP)" to verify the effectiveness of FDN. At the same time, we have also done ablation experiments on FDN to test the constraints imposed necessity.

\subsection{Experimental Setup}
%``Alibaba Click and Conversion Prediction'' 
Ali-CCP is a dataset gathered from real-world traffic logs of the recommender system in Taobao.  This dataset contains click and conversion data. Therefore, it can be used to train MTL models and evaluated by CTR and CVR. In this dataset, the training dataset and the testing dataset have 42 million samples respectively. We sampled the two subsets without replacement, and extracted 40 million data respectively as the experimental sample set. %Note that we did not perform too much feature engineering processing on the original data, but directly used "feature\_id" as the input of the models.
%\chuan{what is a featre\_id? A string or a number? why just use a string or a number as the input?}

%\subsection{Setup}
In the experiment, MMoE and CGC are set with 8 experts, and PLE is set with 2 layers and 16 experts. Our model is set with 2 DCPs for each task.
%When training FDN on Ali-CCP dataset, the batch size and learning rate is set to be 1024 and 0.001 respectively. We set the embedding size as 64 and train the model for 3 epochs. %The model is trained using 4 Tesla P40 GPUs for about 7 hours.
%\chuan{How about the training protocol for other models? Why we use protocol like this? Is this a standard one? If so, you should give some references here.}

\subsection{Experimental Result}

The experimental results are shown in Table~\ref{tab:freq1}. FDN outperforms other models on both CTR and CVR. We also provide the performance of single-task models for comparison. From the results, we can have the following observations: (1) our proposed model achieves the best or second best performance on both tasks; (2) The performance of the MTL model, MMoE, is lower than single-task models, indicating the hard-sharing architecture can limit the model's expressivity; (3) Our model is efficient since it has the least number of parameters. And in order to show how FDN can better decouple task-specific features and task-shared features, We project the features of experts into 2D space and draw the t-SNE\cite{2008Visualizing} diagram (a non-linear dimensionality reduction technique for embedding high-dimensional data into 2D or 3D space for visualization), Fig.~\ref{fig:aliccp-tsne} shows that FDN distinguishes task-specific features and task-shared features more clearly than other SOTA models.
%\chuan{For the t-SNE diagram, you should give a reference and briefly introduce what is t-SNE diagram. I am not sure whether the reviewers in this research field know what t-SNE diagram is.}
%It is worth noting that the number of parameters in FDN is much fewer than the state-of-the-art method PLE. 

\begin{table}[t]
  \caption{Quantitative Results on Ali-CPP Dataset}
  \centering
  \label{tab:freq1}
  \resizebox{0.9\columnwidth}{!}{
  \begin{tabular}{cccccc}
    \hline  Model  & CTR/AUC & CVR/AUC &  \#params \\
    \hline 
    % Single-Task & 0.6189 & 0.6248 & $12.7\times10^{9}$\\
    Single-Task & 0.6189 & 0.6248 & -\\
    MMoE (baseline) & 0.6175 & 0.6239 & $5.75\times10^{9}$\\
    CGC & 0.6235 & 0.6616 & $6.39\times10^{9}$\\
    PLE & 0.6241 & 0.6308 & $7.03\times10^{9}$\\
    FDN (ours) & \textbf{0.6252} & \textbf{0.6783} & $5.11\times10^{9}$\\
    \hline
  \end{tabular}
  }
\end{table}


% \begin{table}[t]
%   \caption{Quantitative Results on Ali-CPP Dataset (offline)}
%   \centering
%   \label{tab:freq1}
%   \resizebox{\columnwidth}{!}{
%   \begin{tabular}{cccccc}
%     \hline  Model  & \multicolumn{2}{c} { CTR/AUC } & \multicolumn{2}{c} { CVR/AUC } &  \#params \\
%     & best & mean & best & mean \\
%     \hline 
%     Single-Task & 0.6196 & 0.6189 & 0.6261 & 0.6248 & $12.7\times10^{9}$\\
%     MMoE (baseline) & 0.6175 & 0.6175 & 0.6239 & 0.6239 & $5.75\times10^{9}$\\
%     CGC & 0.6238 & 0.6235 & 0.6545 & 0.6616 & $6.39\times10^{9}$\\
%     PLE & 0.6244 & 0.6241 & 0.6489 & 0.6308 & $7.03\times10^{9}$\\
%     FDN & \textbf{0.6255} & \textbf{0.6252} & \textbf{0.6778} & \textbf{0.6783} & $5.11\times10^{9}$\\
%     \hline
%   \end{tabular}
%   }
% \end{table}

% \begin{table}[t]
%   \caption{Ablation Study on Ali-CPP Dataset}
%   \centering
%   \label{tab:ablation}
%   \resizebox{0.9\columnwidth}{!}{
%   \begin{tabular}{ccccc}
%     \hline  Model  & \multicolumn{2}{c} { CTR/AUC } & \multicolumn{2}{c} { CVR/AUC } \\
%     & best & mean & best & mean \\
%     \hline 
%     FDN(without aux) & 0.6153 & 0.6151 & 0.6594 & 0.6610 \\
%     FDN(without orth) & 0.6202 & 0.6193 & 0.6619 & 0.6615 \\
%     FDN(without shared-feature) & 0.6168 & 0.6163 & 0.6596 & 0.6658 \\
%     % FDN(1-ensemble) & 0.6213 & 0.6157 & 0.6061 & 0.5709 \\
%     % FDN(2-ensemble) & 0.6221 & 0.6186 & 0.6231 & 0.5940 \\
%     FDN & \textbf{0.6255} & \textbf{0.6252} & \textbf{0.6778} & \textbf{0.6783} \\
%     \hline
%       \end{tabular}
%   }
% \end{table}

\begin{table}[t]
  \caption{Ablation Study on Ali-CPP Dataset}
  \centering
  \label{tab:ablation}
  \resizebox{0.9\columnwidth}{!}{
  \begin{tabular}{ccccc}
    \hline  Model  & CTR/AUC & CVR/AUC \\
    \hline 
    FDN(without aux) & 0.6151 & 0.6610 \\
    FDN(without orth) & 0.6193 & 0.6615 \\
    FDN(without task-shared feature) & 0.6143 & 0.6558 \\
    % FDN(1-ensemble) & 0.6213 & 0.6157 & 0.6061 & 0.5709 \\
    % FDN(2-ensemble) & 0.6221 & 0.6186 & 0.6231 & 0.5940 \\
    FDN & \textbf{0.6252} & \textbf{0.6783} \\
    \hline
      \end{tabular}
  }
\end{table}


\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{AliCCP-t-sne2.pdf}
  \caption{2D space t-SNE feature distributions learned by task-shared experts and task-specific experts of our proposed model in Ali-CCP Dataset.
  %In t-SNE, it is obvious that our proposed FDN decouples task-specific features and task-shared features more obviously than the SOTA models.
  }
%   \Description{decouples task-specific features and task-shared features.}
  \label{fig:aliccp-tsne}
\end{figure}

%The results show that the FDN has good learning ability, reaching the level of the most advanced model, especially CVR, FDN has a strong fitting ability. In addition, the ablation experiment also proved the necessity of constraint design.

\subsection{Abalation Study} We further conducted several experiments to show the contribution of each component in our model. As shown in Table~\ref{tab:ablation}, we remove each component from the full model, including the orthogonal constraint (FDN(w/o orth.)), auxiliary task (FDN(w/o aux.)) and task-shared feature fusion constraint (FDN(w/o task-shared feature.)). %We also verify the effectiveness of the ensemble strategy, i.e., different task-shared experts learn complementary features. So we did comparison experiments where the task-shared features are from only 1 or 2 task-shared experts (FDN(1-ensemble) and FDN(2-ensemble)). 
It is clearly to see that all the component contributes to the final performance to a certain degree.



% \subsection{Xiaomi Radio Dataset}

% %This subsection introduces our experiments on the Xiaomi Radio Recommendation. The purpose of this scenario is to recommend favorite albums for users and improve their play time. We take click and valid play as the object of multi-task learning optimization.

% \subsubsection{Data description}

% %To verify the effectiveness of the proposed model in real-world recommendation scenario, 
% Xiaomi radio is a system app of Xiaomi mobile phone. Our experiment is mainly conducted on the album recommendation channel of Xiaomi radio. This industry dataset was constructed by collecting 320 million user dataset of Xiaomi radio log, including 11 million users and 140000 high-quality albums. According to the time sequence, we divided the dataset into the training set and the verification set by the ratio of 7:3. The main goal of the Xiaomi Radio recommendation scenario is to improve the user's album playing time. Therefore, we take click and valid play as the targets of multi-task learning.

% \subsubsection{Setup}
% The learning rate, batch size, embedding size, and maximum epoch as set to be 0.001, 2048, 32, and 5, respectively.
% % Learning rate, batch size, embedding size, maximum epochs.
% %We take MMoE, the most commonly used multi-task learning model in the industry, as the baseline, and compare it with the state-of-the-art multi-task learning model CGC / PLE. 

% \subsubsection{Evaluation}

% We use AUC as the offline evaluation metric. From Table~\ref{tab:freq2}, it can be seen that our model outperforms all the other models in both the click-through rate and the valid play rate.

% Based on this, we have more online control experiments on ABTest. The experimental data was collected for 7 days. It can be seen from Table~\ref{tab:freq3} that our model has improved both CTR and per-capita playtime (PCP).



% \begin{table}[t]
%   \caption{Quantitative Results on Xiaomi Radio (offline)}
%   \centering
%   \label{tab:freq2}
%   \smallskip
%   \resizebox{\columnwidth}{!}{
%   \begin{tabular}{ccccc}
%     \hline Model & click/AUC & valid play/AUC & \multicolumn{2}{c} { Gain } \\
%     & & & click & valid play \\
%     \hline MMoE(baseline) & 0.7263 & 0.7504 & 0.0 & 0.0 \\
%     CGC & 0.7275 & 0.7554 & +0.0012 & +0.0050 \\
%     PLE & 0.7271 & 0.7518 & +0.0008 & +0.0014 \\
%     FDN & \textbf{0.7297} & \textbf{0.7574} & \textbf{+0.0034} & \textbf{+0.0070} \\
%     \hline
%   \end{tabular}
%   }
% \end{table}
% \begin{table}[t]
%   \caption{Performance Gains Brought by Different Models on Xiaomi Radio (online)}
%   \centering
%   \label{tab:freq3}
%   \resizebox{0.55\columnwidth}{!}{
%   \begin{tabular}{ccc}
%     \hline Model & CTR & PCP \\
%     \hline MMoE(baseline) & $0.00 \%$ & $0.00 \%$ \\
%     \hline CGC & 0.525\% & 0.913\% \\
%     PLE & 0.391\% & 0.494\% \\
%     FDN & \textbf{1.749\%} & \textbf{2.238\%} \\
%     \hline
%   \end{tabular}
%   }
% \end{table}


% \subsection{Census-Income Dataset}

% \subsubsection{Data description}
% Census-Income dataset contains weighted census data extracted from the 1994 and 1995 Current Population Surveys conducted by the U.S. Census Bureau. The data contains 40 demographic and employment related variables. We set `income\_50k' and `marital\_stat' as two labels. This data contains 199523 train dataset and 99762 test dataset.

% \subsubsection{Setup}
% The learning rate, batch size, embedding size, and maximum epoch as set to be 0.005, 1024, 32, and 20, respectively.
% %\chuan{The setup for this dataset is not the same as the setup for Ali dataset. You should give the reason here. Also, what is the training protocol for other competitors?}

% \subsubsection{Evaluation Results}
% Evaluation results on Census-Income Dataset shown in Table~\ref{tab:census-incomeexp} demonstrate that our proposed FDN outperforms the SOTA models on the AUC of two tasks. 

% \begin{table}[t]
%   \small
%   \caption{Evaluation Results on Census-Income Dataset}
%   \centering
%   \label{tab:census-incomeexp}
%   \resizebox{0.9\columnwidth}{!}{
%   \begin{tabular}{ccccc}
%     \hline  Model  & income\_50/AUC &  marital\_stat/AUC \\
%     \hline 
%     %Single Task & 0.0\% & 0.0\% \\
%     MMoE & 0.9432 & 0.9935 \\
%     CGC & 0.9427 & 0.9940 \\
%     PLE & 0.9446 & 0.9943 \\
%     FDN & \textbf{0.9469} & \textbf{0.9945} \\
%     \hline
%       \end{tabular}
%   }
% \end{table}


==> LaTeX 3/IdealExperiment.tex <==
\section{Experiments on Synthetic Dataset}

In the real dataset, due to the complexity of business and the influence of data noise, it is difficult to ideally decompose the original feature input into task specific and task shared features. Therefore, in order to establish the ability of feature decomposition of the models, we use a synthetic data that is easy to verify the decoupling ability of the model.

%In the real dataset, there is a lot of noise in the original input features, so it is difficult to completely decouple these features into task-specific features and task-shared features. Therefore, in order to establish the ability of feature decomposition of the models, we use a synthetic data that is easy to verify the decoupling ability of the model.
%\chuan{The logic here is correct, but the presentation needs to be revised.}

\subsection{Synthetic Dataset Generation}
Inspired by the previous synthetic data in MMOE \cite{ma2018modeling}, we generated two regression tasks (task A and task B) and generated the ideal synthetic features corresponding to two tasks. In addition, we also generated features for two tasks individually to approximate the ideal performance of the tasks by the single task model. Finally, we generated three datasets, namely Dataset-$A$ : [[task A], [data synthesized by shared features and task A specific features]], Dataset-$B$ : [[task B], [data synthesized by shared features and Task B specific features]], and Dataset-$I$ : [[task A, Task B], [data synthesized by shared features, task A specific features and Task B specific features]], where Dataset-$A$ and Dataset-$B$ are to approach the ideal performance of the two tasks by the single task model respectively, and Dataset-$I$ is the ideal data set finally synthesized to verify the feature decoupling ability of MTL. Further details of generating synthetic data are provided in Appendix.
%Specifically, we generate the synthetic data as shown in the appendix ``synthetic data generation''.

% (1) Randomly generated unit vector $u_{1}, u_{2}, u_{s} \in R^{d}$ :
% \begin{equation}
% \left\|u_{1}\right\|_{2}=1,\left\|u_{2}\right\|_{2}=1,\left\|u_{s}\right\|_{2}=1
% \end{equation}

% (2) Given constant $c_{1}, c_{2}, c_{s}$ generate weight vector:
% \begin{equation}
% w_{1}=c_{1} u_{1}, w_{2}=c_{2} u_{2}, w_{s}=c_{s} u_{s}
% \end{equation}

% (3) Randomly generated $x_{1}, x_{2}, x_{s} \in R^{d}$, where $x_{1}^{i} \sim N(-1,0.1), \\ x_{2}^{i} \sim N(1,0.1), x_{s}^{i} \sim N(0,1)$.

% (4) Generate two labels for regression tasks:
% \begin{equation}
% y_{1}=s+w_{1}^{T} x_{1}+\sum_{i=1}^{m} \sin \left(\alpha_{i} w_{1}^{T} x_{1}+\beta_{i}\right)+\epsilon_{1}
% \end{equation}
% \begin{equation}
% y_{2}=s+w_{2}^{T} x_{2}+\sum_{i=1}^{m} \sin \left(\alpha_{i} w_{2}^{T} x_{2}+\beta_{i}\right)+\epsilon_{2}
% \end{equation}
% where $s=w_{s}^{T} x_{s}+\sum_{i=1}^{m} \sin \left(\alpha_{i} w_{s}^{T} x_{s}+\beta_{i}\right), \epsilon_{1}, \epsilon_{2} \stackrel{\text { i.i.d }}{\sim} N(0,0.01)$

% (5) Generate features:
% \begin{equation}
% \begin{aligned}
% X_{1 i}=& \sin \left(\delta_{i}\left(u_{1}^{i} x_{1}^{i}+u_{s}^{i} x_{s}^{i}\right)+\gamma_{i}\right) + \\ & \cos \left(\delta_{i}\left(u_{1}^{i} x_{1}^{i}+u_{s}^{i} x_{s}^{i}\right)+\gamma_{i}\right)+\varepsilon
% \end{aligned}
% \end{equation}
% \begin{equation}
% \begin{aligned}
% X_{2 i}=& \sin \left(\delta_{i}\left(u_{2}^{i} x_{2}^{i}+u_{s}^{i} x_{s}^{i}\right)+\gamma_{i}\right)+ \\ & \cos \left(\delta_{i}\left(u_{2}^{i} x_{2}^{i}+u_{s}^{i} x_{s}^{i}\right)+\gamma_{i}\right)+\varepsilon
% \end{aligned}
% \end{equation}
% \begin{equation}
% \begin{aligned}
% X_{i}=&\sin \left(\delta_{i}\left(u_{1}^{i} x_{1}^{i}+u_{2}^{i} x_{2}^{i}+u_{s}^{i} x_{s}^{i}\right)+\gamma_{i}\right)+ \\ & \cos \left(\delta_{i}\left(u_{1}^{i} x_{1}^{i}+u_{2}^{i} x_{2}^{i}+u_{s}^{i} x_{s}^{i}\right)+\gamma_{i}\right)+\varepsilon
% \end{aligned}
% \end{equation}
% where $\varepsilon \stackrel{\text { i.i.d }}{\sim} N(0,0.01)$ , $X_{1 i}$ and $X_{2 i}$ as a feature of the single task model, $X_{i}$ as a feature of multitasking dataset.

% (6) Repeat (3), (4) and (5) until enough data are generated.
% %\chuan{If we do not have much space here, we need to move the generation procedures to supplementary materials.}

Since we have generated the dataset of shared features and the specific features of tasks A and B, it is easy to approximate the ideal performance of the tasks. We train the MTL models in the comprehensive synthetic dataset to compare the gap between the ideal performance and results of these MTL models.
%, so as to illustrate the performance of the MTL models. 
%\chuan{Presentation needs to be revised.}

\subsection{Performance on Synthetic Data}
We have repeated experiments in the synthetic data for the proposed FDN and the current SOTA multi-task model, and the model hyper-parameters are same in all experiments. We set the embedding size and the number of experts to be 32 and 8 (FDN has 4 pairs of DCPs), the maximum epoch is 5. Each expert network consists of two fully-connected layers (128 units and 64 units).
% We have repeated experiments in the synthetic data for the proposed FDN and the current SOTA multi-task model, and the model hyper-parameters are same in all experiments.The detailed hyper-parameter settings are as follows: \begin{itemize}
%     \item embedding\_size: 32
%     \item number of experts: 8 (FDN has 4 pairs of DCPs)
%     \item epoch: 5
%     \item expert architecture: 2 layer MLP (128 units and 64 units)
% \end{itemize}
%\textcolor{red}{In addition, we used the single task model to obtain the oracle results of these tasks.}

%\subsubsection{Results}
Mean Square Error (MSE) is used as the evaluation metric.
%, and take the average value of multiple experiments as the experimental results. 
Table~\ref{tab:idealexp} compares the gap between results achieved by each model and oracle results.
%results between each model and the oracle model. 
It is clear to see that our proposed FDN model significantly outperforms other baseline methods.

\begin{table}[t]
  \caption{Performance Gap on Synthetic Dataset}
  \centering
  \label{tab:idealexp}
  \resizebox{0.9\columnwidth}{!}{
  \begin{tabular}{ccccc}
    \hline  Model  & Task A/GAP & Task B/GAP \\
    \hline 
    Oracle Results & 0.0\% & 0.0\% \\
    MMoE & -0.2896\% & -0.3166\% \\
    CGC & -0.0580\% & -0.1981\% \\
    PLE & -0.0433\% & -0.0695\% \\
    FDN (ours) & \textbf{-0.0203\%} & \textbf{-0.0367\%} \\
    \hline
      \end{tabular}
  }
  \vspace{-0.5cm}
\end{table}

==> LaTeX 3/Introduction.tex <==
\section{Introduction}
The recommendation system (RS) is an effective tool to help users to handle \textit{information overload}. It has been widely used in many commercial fields, such as advertising computing, social networks, and e-commerce\cite{wen2019multi}. 
% The recommendation algorithm is the core of RS and directly affects its performance. Traditional recommendation algorithms \cite{liu2015convolutional,guo2017deepfm,zhou2018deep} normally optimize for a single objective.
% Take advertisement recommendation as an example,
% For example, in the application of recommendation, 
% algorithms take the Click-Through Rate (CTR) as the only objective, aiming to predict users' probability of clicking on a specific item. However, in many real-world recommendation applications, user satisfaction is determined by many factors, e.g. clicking, favoriting, sharing and commenting in information recommendation.
%involves the user clicking on the recommended item \textit{and} placing an order on it. 
% Therefore, a single-task model cannot well handle such recommendation problems in practice. Moreover, when multiple tasks are highly correlated, they can mutually benefit each other for feature learning~\cite{torrey2010transfer}, which can improve the performance of each task.
%the knowledge shared between them can be a good guidance for feature learning \cite{torrey2010transfer}, which is conducive to the learning performance of the model.
To improve the user experience, the idea of using multi-task learning (MTL) to satisfy user requirements from multiple aspects has become increasingly popular in the RS community. Many deep learning (DL) based MTL models \cite{ma2018modeling,tang2020progressive} have been proposed for RS. 
However, there is no explicit constraint to force these experts to extract features as required. As a result, the features captured by different experts may still be a mixture of the task-specific feature and the task-shared feature (as shown in Fig.~\ref{fig1}-(a)), which is called \textit{feature redundancy} phenomenon in this paper and will degrade the effectiveness of the model in handling the issue of negative transfer. In the ideal case (as shown in Fig. 1-(b)), feature
spaces should be more pure.
% For example, Ma \textit{et al.} proposed the influential Multi-gate Mixture-of-Experts (MMoE) model \cite{ma2018modeling}. In particular, MMoE leverages expert networks to extract features from the original input and then uses several gating networks to guide feature fusion, where the fused feature can be used for different tasks. However, in MMoE, all tasks share the same expert networks, which model recommendation problems do not always lead to performance improvement, and sometimes even deteriorate the performance of each task. That phenomenon is called \textit{negative transfer}. %As a result, the information represented by the extracted features is limited.
% the expressivity of the extracted features is limited.  
%In fact, MTL can be regarded as a special type of transfer learning, which transfers representations among different yet related tasks to boost all tasks' performance. % However, using MMoE to model recommendation problems does not always lead to performance improvement, and sometimes even result in the performance degradation of each task. %%
% degrades the performance of each task.
%Generally, the features used for each task can be divided into two main categories: task-shared features (shared with other tasks), and task-specific features. \chuan{From my understanding, features shared with other tasks are cross-task features you mentioned in the follow-up content, and features private to themselves are task-specific features. If so, you should mentioned those terms here.}

%However, the task-specific features corresponding to different tasks may mix up during the process of joint training \chuan{what does `mix up' mean here?}. The cross-task feature interference may deteriorate the performance \chuan{what is `cross-task feature interference'? you mean `task-specific feature interference'?}. We call the phenomenon that one task's performance is improving while the other one is dropping \chuan{this sentence needs to be revised. we do not call the phenomenon. you shoud say that the phenomenon that xxxx is observed.}, or all tasks' performance becomes inferior in an MTL model as \textit{negative transfer}. 

%It can be caused by the following reasons. First, when all tasks share the shallow-layers' features, e.g., the experts are shared in MMoE, the expressivity of the extracted features is limited. Second, the feature used for each task can be roughly divided into two parts, features shared with other tasks and features private to themselves. However, the task-specific features corresponding to different tasks may mix up during the process of joint training. The cross-task feature interference may deteriorate the performance. We call the phenomenon that one task's performance is improving while the other one is dropping, or all tasks' performance becomes inferior in a MTL model as \textit{negative transfer}. 

% Researchers have made some attempts to address the issue of negative transfer by improving feature representation ability of MMoE. Tang et al. \cite{tang2020progressive} introduced the Progressive Layered Extraction (PLE) model. In PLE model, expert networks are divided into two groups, i.e., task-specific experts and task-shared experts, and they are designed to extract these two types of features respectively. This model has achieved impressive performance. However, there is no explicit constraint to force these experts to extract features as required. As a result, the features captured by different experts may still be a mixture of the task-specific feature and the task-shared feature (as shown in Fig.~\ref{fig1}), which is called \textit{feature redundancy} phenomenon in this paper and will degrade the effectiveness of the model in handling the issue of negative transfer.
%上述详细解释一下：虽然PLE模型将专家网络分为任务共享和任务特有，但仅仅是通过是否共享某些专家网络实现，并没有一些约束策略，这就导致在模型迭代的过程中，不可避免存在共享特征空间可能包含一些不必要的特定于任务的特征，而一些可共享的特征也可能混合在私有空间中，存在特征冗余现象，如图一所示。

This paper proposes a novel multi-task learning method for recommendation system, named \textbf{F}eature \textbf{D}ecomposition \textbf{N}etwork (FDN). The key idea is to reduce features redundancy by decomposing them with \textit{explicit} constraints. Specifically, we introduce a \textbf{D}e\textbf{C}omposition \textbf{P}air (DCP) to capture task-shared features and task-specific features, respectively. 
% This module consists of a pair of expert networks, aiming for capturing task-shared features and task-specific features, respectively. To ensure the features extracted by the paired expert networks to be decomposed, 
% three constraints are presented: orthogonal constraint, auxiliary task constraint and task-shared feature constraint. 
%Besides, we also adopt the ensemble learning strategy and apply it to improving the representation capability of the extracted task-shared feature without increasing of the numbers of parameters. 
We conducted experiments on a public datasets (i.e., Ali-CCP dataset) to demonstrate the effectiveness of our proposed FDN. %\textcolor{red}{We also provided ablation studies to show the benefit of each component. }

% The contributions of this work are three-fold.
% \begin{itemize}
%   \item [1]
% A new multi-task learning method is proposed for recommendation systems, which can effectively alleviate the issue of negative transfer.       
%   \item [2]
% A novel feature decomposition module is introduced, accompanied by three carefully-designed constraints, to facilitate the expert networks learn the corresponding features.
%  %The method's core idea is to decompose the task-private and task-shared features of multi-tasks with several carefully-designed constraints.
%   \item [3]
% %通过在模型中设置了一些约束策略，抑制了任务共享专家网络和任务特有专家网络中的特征冗余的现象，进一步缓解了多任务学习模型负迁移的问题。通过实验观察，我们的模型超过了目前已有的最先进的多任务学习模型%
% %Our model is simple but effective. It has a simpler architecture with fewer parameters compared with other state-of-the-art (SOTA) models, but can still outperform those methods on both a public dataset and real-world industry datasets. \chuan{Presentation of this paragraph needs to be revised.}
% Extensive experiments have been conducted to demonstrate the effectiveness of the proposed method. Although with fewer parameters, our proposed method achieves the new state-of-the-art (SOTA) performance on both  public dataset and real-world industry datasets.
% \end{itemize}

\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{1_.pdf}
  \vspace{-0.3cm}
  \caption{The green rectangle indicates the task-specific features of Task A, the blue triangle indicates the task-specific features of Task B, and the pink circle indicates task-shared features.
  %In MTL, task features are divided into task-specific features and task-shared features. As shown in (a), the current SOTA model explicitly devided experts into task-shared experts and task-specific experts. Due to the lack of explicit constraints on experts, there may be a specific feature space including other features, that is, the so-called feature redundancy, which may lead to the problem of negative transfer. In the ideal case (as shown in Figure b), feature decomposition should be more pure. The feature space of each expert should contain the features corresponding to the current expert, rather than other features, which will lead to better performance.
  %In MTL, task features are divided into task-specific features and task-shared features. As shown in (a), features learned for each task by the current SOTA methods \cite{tang2020progressive} may be impure as they learn such decomposition implicitly. In contrast, with our proposed constraints, the features can be effectively decomposed into task-shared and task-specific features, as shown in (b). The decomposed features are purer thereby the features for each task will be more representative, leading to better performance.
  %as task-specific features without related constraints, in the current SOTA models, task-shared features may contain unnecessary features, while task-specific features may contain unnecessary features, suffering from \textit{feature interference}. 
  %The negative transfer problem in multi-task learning. Given the original input (grey box), a MTL model extracts features for different tasks (e.g., A and B). As shown in (b), it is assumed that some features (e.g., circles) are shared by different tasks while some are private (e.g., green rectangles are specific for Task A while the blue triangles are for Task B). However, in (a), these private features are mixing up, which could be harmful for task performance.
  }
%   \Description{negative transfer.}
    % \vspace{-0.5cm}
  \label{fig1}
\end{figure}





==> LaTeX 3/Method.tex <==
%\section{Multi-task learning model with multiple constraint losses}
\section{Methodology}

\subsection{Feature redundancy in  MTL}

%In RS, MTL has been applied to many services, but due to the impact of negative transfer, MTL can not improve the performance of all tasks at the same time, which is also one of the current research directions. Many researchers have began to notice this problem and to solve it. 
The negative transfer in MLT is considered to be caused by the fusion of expert's features. Therefore, by explicitly dividing the expert networks into task-shared experts and task-specific experts, PLE \cite{tang2020progressive} model can alleviate the problem of negative transfer. % caused by feature fusion. 
However, explicit expert network division strategy can not completely solve the problem. % of negative transfer. 
As shown in Fig.~\ref{fig1}-(a), due to the lack of explicit constraints on experts, there may be a specific feature space including other spaces' features, that is the so-called feature redundancy. Due to the above phenomena, there will be task-specific features in the task-shared feature space or task-specific features of other tasks in the current task-specific feature space, which will weaken the representation ability of MTL and lead to the problem of negative transfer. In the ideal case (as shown in Fig.~\ref{fig1}-(b)), feature spaces should be more pure. To solve the phenomenon of feature redundancy, we propose DCPs.
%The feature space of each expert should contain the features corresponding to the current expert, rather than other features, which will lead to better performance. To solve the problems, we propose DCPs to solve them.

% In RS, MTL has been applied to many services, but due to the impact of negative transfer, MTL can not improve the performance of all tasks at the same time, which is also one of the current research directions. Many researchers have begun to notice this problem and begin to solve it. The negative transfer in MLT is considered to be caused by the fusion of task-specific features and task-shared features. Therefore, by explicitly dividing the expert network into task-shared experts and task-specific experts, PLE \cite{tang2020progressive} model can alleviate the problem of negative transfer caused by feature fusion. However, explicit expert network division strategy can not completely solve the problem of negative transfer, because divided expert networks do not have some constraint strategies to induce them to learn the feature information in the corresponding domain, and there will be the phenomenon of task-shared features mixed in the task-specific feature domain or task-specific features mixed in the task-shared feature domain, which is called feature redundancy. To solve these problems, we propose DCPs to solve them.

\subsection{Preliminaries}

%In principle, our proposed FDN model is a general MTL model, which can be applied in many practical scenarios. In this work, we mainly focus on the recommendation application. 
%
Given $K$ tasks (e.g., clicking, sharing, etc), the corresponding labels are $\left\{y_{1}, \ldots, y_{K}\right\}$. $X \in R^{n}$ denotes the input representation where $n$ refers to the dimension of the input. 
%Then the sample set can be represented as $\left\{ y_{1}, \ldots, y_{K}\mid X \right\}$, 
The predictions of the $k$-th task can be expressed as $\hat{y}_{k}=f^{MTL}_{k}(X)$,
where $f^{MTL}_{k}(\cdot)$ refers to the network for the $k$-th task of a multi-task learning model.

% 这里的特征解耦模块，改成解耦对（decomposition pairs, DCP）,另外encoder应该需要跟之前的论文保持一致为expert。
As shown in Fig.~\ref{fig:architecture}, FDN consists of multiple newly-proposed decomposition pairs (DCPs). For each task, there are $M$ DCP modules. Each DCP module has a pair of experts, a task-specific expert and a task-shared expert. Task-specific expert, which is denoted by $f^{p}$, captures features which are specific for each individual task. Task-shared expert is denoted by $f^{s}$, which extracts features that are potentially shared by all the tasks. After extracting the decomposed features, the model then fuses these features and feeds the features into prediction layer of each task. The process can be represented as follows:

\begin{equation}
f^{MTL}_{k}(X)=\sigma(g_{k}(f^{p}(X),f^{s}(X)))
\label{eq:fdn}
\end{equation}
where $g_{k}(.)$ is a fusion function for task $k$ and $\sigma$ is an activation function.
%Like the previous work, we ch onstruct the loss function of task output. We require the model to generate the optimal solution of each task after training:
%\chuan{From the above paragraph, you just describe how you design the model, but you do not explain why you design the model like this. In an ideal way, you should give a reason for each model design.}
Next, we will explain these constraints applied to obtain the decomposed features.

\begin{figure*}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{2_.pdf}
  \caption{Architecture of the proposed Feature Decomposition Network: 
The gray rectangle box represents the original input, each DeComposition Pair (DCP) consists of two expert networks, including a task-shared expert network (pink box) and task-specific expert network (green or blue box). The detail of the DCPs is shown in the dashed box. An auxiliary task head is added for each DCP to promote feature decomposition.}
%the light green and blue rectangle boxes represent the DeComposition Pairs (DCPs) for task A and task B respectively. The pink rectangle denotes task-shared features. The detail of DCP is shown in the dashed box: the small pink rectangle is task-shared expert, the small light blue rectangle is task-specific expert, and the rounded rectangle represents the auxiliary task (task B in this figure).% \chuan{The captions for Figures 1 and 2 are too long. The detailed descriptions could be moved to the main content.}}
%   \Description{Model Architecture.}
  \label{fig:architecture}
\end{figure*}

\subsection{DeComposition Pair}

As explained before, negative transfer is caused by feature redundancy. To address this problem, our idea is to reduce such redundancy by \textit{explicitly} decomposing features into task-specific and task-shared features. Such design will make the model recombine features based on the requirements of each task. Three constraints are introduced into DCP module.

%The novelty of our model is to solve the negative transfer problem mentioned in Section 2. On the basis of the previous work, our model (as shown in Fig \ref{fig2}) is composed of several modules. Each module takes the original feature as input, and the output is taken as part of the main task input after module processing. The proposed module is composed of two feature encoders, one is used to extract task-specific features, named task-specific-encoder, and the other is used to extract task shared features, named task-shared-encoder, each encoder is a multi-layer perceptron that can specify the number of layers and neurons. In addition, it should be pointed out that we can set a different number of modules for each task through hyper-parameter. To achieve the model structure, we have designed some constraints. Next, we will introduce these constraints in detail.

\subsubsection{Orthogonal Constraint}
Orthogonal constraint has been widely explored for feature decomposition \cite{wan2019generative,salzmann2010factorized,salzmann2010factorized,bousmalis2016domain}. In order to decompose the original features into task-specific features and shared features as much as possible, we add the orthogonal constraint between the extracted features of the two experts. The orthogonal constraint is represented as follows:
%We add the orthogonal constraint between the extracted features of the two encoders. The orthogonal constraint is represented as follow:

\begin{equation}
L_{\text {orth}}=\sum_{k=1}^{K} \sum_{m=1}^{M}\left\|\left(f_{m}^{s}\right)^{\top} f_{m}^{p}\right\|_{F}^{2}
\end{equation}
where $M$ denotes the number of modules of task $k$, $f_{m}^{s}$ denotes the feature extracted by the $m$-th task-shared expert of tash-$k$, and $f_{m}^{p}$ is from the $m$-th task-specific expert of tash-$k$. $\|\cdot\|_{F}^{2}$ denotes squared Frobenius norm.

\subsubsection{Auxiliary Task Constraint}
Orthogonal constraint can help experts capture complementary features, but not necessarily decompose the features into task-shared and task-specific. Therefore, in order to capture task-specific features, we introduce an auxiliary task to each task-specific expert as a regularizer. Specifically, we treat each task-specific expert as a single-task network and directly use its extracted feature for the prediction of a specific task (as shown in  Fig.~\ref{fig:architecture}(Right) rounded rectangular box marked with "aux" text). Such design can induce the task-specific expert to extract the most salient task-specific feature for the current task. It is worth noting that the auxiliary task objective is the same as the final loss of the task. Thus, the corresponding labels are the same. It can be represented as follows:
%\chuan{The presentation of this paragraph needs to be revised.}

%In order to enhance the ability of task-specific encoder to extract features, we design auxiliary task loss constraint. In single-task learning, some salient features have a great influence on the learning results. We use the constraint of auxiliary task to extract the task-specific feature, which is similar to single-task learning. Our model quickly extract the salient features of the current task from the original input, that is, the task-specific features. At the same time, in the current task-specific feature extraction process, it avoids the mixing of shared features or other task-specific features, and effectively reduces the negative transfer problem in multi-task learning \cite{liu2018decoupled,zhang2017survey}. It should be pointed out that our auxiliary task loss function is the same as the final output loss function of the task:

\begin{equation}
L_{aux}=\sum_{k=1}^{K} \sum_{m=1}^{M} L_{k,m}\left(\hat{y}_{m}^{k}, y^{k}\right)  
\end{equation}

\begin{equation}
\hat{y}_{m}^{k}=\sigma(f_{m}^{k,p}(X))
\end{equation}
where $L_{k,m}(\cdot)$ is the $k$-th auxiliary task loss, and $\hat{y}_{m}^{k}$ denotes the prediction result of using the extracted feature of the $m$-th task-specific expert.

\subsubsection{Task-shared Feature Fusion Constraint}
These task-shared experts of different DCPs can be treated as an fusion model which is able to extract more expressive features than the model using the shared parameters. The fusion of task-shared experts in DCPs is equivalent to a constraint, which will induce the model to further learn task-shared features. Once obtaining the decomposed features, the model fuses these features by concatenation ($g_{k}(.)$ in Eq.~\ref{eq:fdn}), as shown in Fig.~\ref{fig:architecture}.

%The task-shared experts of different DCPs share the same architecture but different parameters. Therefore, these task-shared experts can be treated as an fusion model which is able to extract more expressive features than the model using the shared parameters. Once obtaining the decomposed features, the model fuses these features by concatenation ($g_{k}(.)$ in Eq.~\ref{eq:fdn}), as shown in Fig.~\ref{fig:architecture}.
%Because the experts' architectures are simple, such design will only slightly increase the number of parameters. 

%Once obtaining the decomposed features, the model fuses these features by concatenation ($g_{k}(.)$ in Eq.~\ref{eq:fdn}), as shown in Fig.~\ref{fig:architecture}. The concatenation operation can be replaced by other fusion operations such as element-wise addition or gating mechanism as in \cite{ma2019snr}. We empirically found that simple concatenation can already produce satisfactory results due to the strong representation capability of the output features produced by DCP.% \chuan{expressivity -> representation capability? You can add something like "as observed in Section XX".}

%After the previous design, we do not use tower to mine the extracted features in a deeper level, and directly merge and concatenate them as the multi-task input. This is because, after imposing constraints on the encoders, the generated features are already significant enough for the expression of the task, and further mining may cause information loss.

\subsubsection{Total Loss and Implementation Details}

The final loss function of our model is defined as $L=L_{\text {task }}+L_{\text {orth }}+L_{\text {aux }}$.
% \begin{equation}
% L_{\text {task}}=\sum_{k=1}^{K} \lambda_{k} L_{k}\left(y_{k}, \hat{y}_{k}\right)
% \end{equation}
% where $\lambda_{k}$ is the hyper-parameter of the model, denoting the weight of the loss function of each task output. $L_{k}(\cdot)$ is the loss function of task $k$. 
% In our implementation, each encoder consists of \textcolor{red}{explain architecture of encoders}. 
%For simplicity, in our implementation, each expert consists of a multi-layer perceptron (MLP) with two fully-connected layers, and this improves the efficiency of the model in the inference stage. In addition, we did not use the tower for further feature extraction as used in MMoE / CGC / PLE, which reduces the amount of parameters, and, as explained before, features of DCP already have sufficient expressive ability and thus it is unnecessary to use additional towers.
%\chuan{You need to give some justifications why you implement the model like this.}
For fair comparison, in our implementation, the expert of DCP is designed to be feed-forward network the same as that of MMOE. In addition, in the architecture of MMoE, CGC, and PLE, the design of the tower network is mainly to eliminate the influence of noise on the model performance. In our proposed model, we did not use the tower network as used in MMoE, CGC, PLE, which reduces the amount of parameters, and, as explained before, DCPs have solved the problem of feature redundancy at the expert level and the feature fusion module (as shown in Fig.~\ref{fig:architecture}) has been used to eliminate the noise in advance, thus it is unnecessary to use additional tower networks.

==> LaTeX 3/Related.tex <==
\section{Related works}

%\subsection{Multi-task learning in Recommendation}

% \textcolor{red}{check this part in the PLE paper and include more related works}
In recent years, many MTL models have been proposed for RS. Except for the aforementioned MMoE and PLE, Ma et al. \cite{tang2020progressive} proposed the Entire Space Multi-task Model (ESMM). This model uses features provided by CTR and click- through\&conversion rate (CTCVR) to help build Conversion rate (CVR) model in the whole output space. However, due to the diversity of optimization target types and the number of tasks (generally more than two tasks), ESMM will have the following problems: 1) ESSM cannot easily support other tasks besides classification tasks; 2) With the increase of the number of tasks, ESMM has poor scalability. 

Besides, there have also been some works utilizing AutoML strategy to find a good network structure. Ma et al. \cite{ma2018entire} proposed Sub-Network Routing (SNR) to improve the performance with a flexible parameter sharing strategy by using a routing network. SNR controls sub-networks inputs of each task by binary variables and apply Neural Architecture Search (NAS) strategy to search network structure. Influenced by SNR, Ding et al. \cite{2021MSSM} proposed the multiple level sparse sharing model (MSSM). MSSM proposed field-level and sell-level sparse connection module by binary variables. However, this strategy requires a lot  of parameters, which can be a burden when deploying the model online.
%In recommendation, due to good performance and multi-dimensional description of business, multi-task learning has attracted great attention in the industry.

%Xiao Ma et al. \cite{tang2020progressive} proposed Entire Space Multi-task Model(ESMM), which uses the features provided by CTR and click- through\&conversion rate (CTCVR) to help build Conversion rate(CVR) model in the whole output space. However, due to the diversity of optimization target types and the number of tasks (generally more than two tasks), ESMM will have some problems: 1) ESSM cannot easily support other tasks besides classification tasks; 2) With the increase of the number of tasks, ESMM model has poor scalability.

%Jiaqi Ma et al. \cite{ma2018modeling} proposed Multi-gate Mixture-of-Experts (MMoE), which is based on the ensemble of subnets and uses multiple experts for multi-task learning. But MMoE is a hard-parameter sharing model, namely, each task shares a common experts layer, which limits the ability of the model to express the specific information of each task.

%Jiaqi Ma et al. \cite{ma2018entire} proposed Sub-Network Routing (SNR), which decomposes the whole neural network model into some sub-networks, and then realizes flexible parameter sharing by sub-network routing, so as to improve the accuracy of multi-task learning model. However, this strategy needs a large number of parameters to implement, resulting in the increase of model parameters, which is not conducive to the online deployment of the model.

%\textcolor{red}{\subsection{Negative Transfer in Multi-task learning} This may be duplicate to the introduction}

%With the large-scale application of multi-task learning in RS, we find that multi-task learning has a negative transfer problem. Based on MMoE, Hongyan Tang et al. \cite{tang2020progressive} assign different roles to different experts to alleviate the issue of negative transfer. However, this can not completely solve the problem. This may be because when the model performs feature transformation on the original input, it only takes a corresponding strategy for parameter sharing, and does not explicitly disentangle the original features, resulting in that after multiple iterations, the task-specific space still contains the shared features, and the shared feature space still contain some task-specific features. Due to improper mixture of features, the expression ability of the model is damaged, which causes the so-called negative transfer (as shown Fig \ref{fig1} ). Therefore, we deal with this problem via the idea of explicit feature decomposition.

% \textcolor{red}{1. which work points out this problem for the first time? 2. what reasons cause this problem? 3. what strategies or algorithms have been proposed to handle this problem?}


